From Online Behaviours to Images: A Novel Approach to Social Bot Detection

Online Social Networks have revolutionized how we consume and share information, but they have also led to a proliferation of content not always reliable and accurate. One particular type of social accounts is known to promote unreputable content, hyperpartisan, and propagandistic information. They are automated accounts, commonly called bots. Focusing on Twitter accounts, we propose a novel approach to bot detection: we first propose a new algorithm that transforms the sequence of actions that an account performs into an image; then, we leverage the strength of Convolutional Neural Networks to proceed with image classification. We compare our performances with state-of-the-art results for bot detection on genuine accounts / bot accounts datasets well known in the literature. The results confirm the effectiveness of the proposal, because the detection capability is on par with the state of the art, if not better in some cases.

==> sections/cnns.tex <==
\section{Convolutional Neural Networks}\label{sec:cnn}
{\bf mari: non rivedo questa sezione, ma a una letta veloce direi di stringare molto....}
In this section, we want to provide an overview of Convolutional Neural Networks (CNNs), which are well-suited for image and video analysis and, in particular, for tasks such as object recognition, face recognition, and image segmentation. Given the recent and noteworthy \cite{CNNAdvancements, sultana2018advancements} advancements in the field of Convolutional Neural Networks, we asked ourselves whether these networks could be used to classify Twitter accounts into bot / human.

CNNs are typically composed of three layers: convolutional layers, pooling layers, and fully connected layers. The convolutional layer is the fundamental component of a CNN and it requires most of the computation. The input is an image and the dimension of the input image changes depending on whether it is grayscale or colored. If it is grayscale, the input will have one dimension, while if it is colored, it will have three dimensions (representing the RGB values). Combined with the convolutional layer, there is the ``filter'' or ``kernel''  which is a matrix of small size. From the convolution operation, we have in output a ``filtered'' image which is a sequence of dot products between the input pixels and the kernel. Afterward, an activation function (i.e. the Rectified Linear Unit -- ReLU) can be applied to the output. It is also possible to optimize the convolution layer through some hyperparameters, such as the ``stride'' and the ``padding''. The former represents the amount of movement of the kernel over the input, while the latter is the process of padding the border of the input. When we add zeros as padding, we refer to ``zero-padding''.
The second type of layer is the ``pooling'' layer. A pooling layer is used to downsample the given input. There are two main types of pooling: max-pooling and average-pooling. In the first case, the function selects the maximum value between the pixels that the kernel is considering. In the second case, it calculates the average value between the pixels and sends it to the output.
The third type of layer is the ``Fully-Connected'' (FC) layer, also known as a ``dense'' layer. The neurons in a FC-layer receive input from all the neurons in the previous layer. Usually, FC-layers exploit the softmax activation function to classify the inputs and to produce the real classification.

In this study, we employed the transfer learning, allowing us to utilize pre-trained models rather than starting from scratch. We tried several models, such as the VGG16, EfficientNet, Inception, ResNet50, and WideResNet50. In \autoref{sec:exp-res} we will report the best results, which were obtained from the models of the ResNet family.
 
%The approach proposed in this study uses the \textit{Convolutional Neural Networks} (CNNs). These CNNs had remarkable advancements in recent years, which is why they are exploited in the study.
%These types of networks make use of different layers. The first type of layers is the convolutional layer, which uses convolution, a mathematical operation described in the \autoref{eq:discrete_convolution}.

%\begin{equation}
%f[m, n] = \sum_{k, l} I[m - k, n - l]g[k, l]
%\label{eq:discrete_convolution}
%\end{equation}

%In \autoref{eq:discrete_convolution} $f$ will be the ``filtered" image, and $I$ is the image given in input to the layer. The function $g$ represents the kernel, a small matrix used, for example, to blur the image in input.
%When a convolutional layer processes the input, it is possible to add a number of pixels; this is the padding. In addition to the padding, it is possible to specify the stride parameter, which represents the amount of movement over the input. The following formula gives the size of output from a convolutional layer:
%\begin{equation}
%W_{out} = \frac{W - K + 2P}{S} + 1
%\label{eq:w_out}
%\end{equation}
%In \autoref{eq:w_out}, $W$ is the width (or the height if $W = H$), $K$ is the kernel size, $P$ is the padding, and $S$ is the stride.

%Another type of layer used in these networks is the pooling layer. These are used to downsample the given input, and different pooling functions can be used in this step.

%In a CNN, the last layer is a fully connected layer in which all the neurons are linked.

%Another technique used in this study is transfer learning. Training a CNN from scratch, initially with random weights, is difficult since it requires high-performance hardware. To avoid the step of training from scratch, it is common to use some pre-trained networks on a huge dataset such as ImageNet \cite{deng2009imagenet}, which has more than 1 million images and 1000 different categories.
%In this work, the transfer learning technique was used in two ways:
%\begin{itemize}
%    \item fixed feature extractor: in this case, the last fully connected layer of the network is replaced by a layer that has in input the number of features in output from the previous layer and 2 (the number of classes needed). The weights are frozen for all the layers except for the last one;

%    \item fine-tuning: this is similar to the previous one, but here some of the weights are not frozen and are "fine-tuned" during the training on the custom dataset.
%\end{itemize}

%However, there are no substantial differences in the achieved results with respect to the technique used.

==> sections/digital-dna.tex <==
\subsection{Digital DNA}\label{sec:digitalDNA}
The biological DNA contains the genetic information of a living being and is represented by a sequence which uses four characters representing the four nucleotide bases: A (\textit{adenine}), C (\textit{cytosine}), G (\textit{guanine}) and T (\textit{thymine}). Digital DNA is the counterpart of biological DNA and it encodes the behaviour of an online account. In particular, it is a sequence consisting of $L$ characters from a predefined alphabet $\mathbb{B}$: 
% The latter is formally defined as $\mathbb{B}$ and it contains different symbols; mathematically $\mathbb{B}$ is defined as follows:
\begin{equation}
\mathbb{B} = \{\ \sigma_1, \sigma_2, \sigma_3, ..., \sigma_N \}, \; \sigma_i \neq \sigma_j \: \forall i, j = 1, ..., N \: \land i \neq j
\label{eq:digitalDNA}
\end{equation}

In \autoref{eq:digitalDNA} each $\sigma$ is a symbol of the alphabet and a digital DNA sequence will be defined as follow:
\begin{equation}
s = (\sigma_1, \sigma_2, ..., \sigma_n), \; \sigma_i \in \mathbb{B} \; \forall \; i = 1, ..., n
\end{equation}
Each symbol in the sequence denotes a type of action. In the case of Twitter, a basic alphabet is formed by the 3 actions representing the types of tweets:
\begin{equation}
%\mathbb{B}^{3}_{\text{type}} = 
\mathbb{B} = \left\{\begin{array}{c}
        A = \text{tweet}, \\
        C = \text{reply}, \\
        T = \text{retweet}
        \end{array}\right\}
        \label{eq:alphabetExample}
\end{equation}
According to the type of tweets, it is thus possible to encode the account timeline, which could be, e.g., the 
following $s = ACCCTAAACCCCCCTT$. 

Strings of digital DNA were compared to each other in~\cite{Cresci2018fingerprinting}: the longer the \textit{longest common substring} of a group of accounts, the more likely that group is made up of accounts programmed to complete a similar task, i.e., the more likely those accounts are automated accounts.



% In this way, the account information is represented by a compact notation. Then, in \cite{cresci2017} the authors leveraged the LCS (\textit{longest common substring}) curves to detect social spambots. They reached excellent results, like $MCC$ of $0.952$ and $0.955$ on a dataset with genuine accounts and retweeters of the political candidate, and $MCC$ of $0.867$ and $0.940$ on a dataset with genuine accounts and spammers of \textit{Amazon} products.

